A Double Machine Learning Approach for the Evaluation of COVID-19 Vaccine Effectiveness under the Test-Negative Design: Analysis of Qu\'ebec Administrative Data

The test-negative design (TND), which is routinely used for monitoring seasonal flu vaccine effectiveness (VE), has recently become integral to COVID-19 vaccine surveillance, notably in Qu\'ebec, Canada. Some studies have addressed the identifiability and estimation of causal parameters under the TND, but efficiency bounds for nonparametric estimators of the target parameter under the unconfoundedness assumption have not yet been investigated. Motivated by the goal of improving adjustment for measured confounders when estimating COVID-19 VE among community-dwelling people aged $\geq 60$ years in Qu\'ebec, we propose a one-step doubly robust and locally efficient estimator called TNDDR (TND doubly robust), which utilizes cross-fitting (sample splitting) and can incorporate machine learning techniques to estimate the nuisance functions and thus improve control for measured confounders. We derive the efficient influence function (EIF) for the marginal expectation of the outcome under a vaccination intervention, explore the von Mises expansion, and establish the conditions for $\sqrt{n}-$consistency, asymptotic normality and double robustness of TNDDR. The proposed estimator is supported by both theoretical and empirical justifications.

==> Sections/test.tex <==


\section{An additional derivation about the EIF of $\psi_v$}
In the preceding section, we established the EIF of $\psi_v$ by incorporating debiasing weights in the form of a propensity ratio. In the subsequent process of deriving the EIF, we will utilize an alternative type of debiasing weights that
\begin{equation*}
     \omega_v(\boldsymbol{c}) = \frac{ \mathbb{P}_{TND}(Y = 0\mid  \boldsymbol{C}  = \boldsymbol{c} )}{\mathbb{P}_{TND}(Y = 0 \mid V=v ,  \boldsymbol{C}  = \boldsymbol{c} )} := \frac{m^0(\boldsymbol{c})}{\mu^0_v(\boldsymbol{c})}.
\end{equation*}
Using influence function building blocks, namely the EIF of $\mathbb{P}_{TND}(Y = 1 \mid X = x)$ in Equation (\ref{EIFmodel}), we have
\begin{equation*} 
     \mathbb{EIF}(m^0(\boldsymbol{c})) = \frac{\mathbb{I}\left(Y = 0, \boldsymbol{C}  = \boldsymbol{c}\right)-\mathbb{I}\left(\boldsymbol{C}  = \boldsymbol{c}\right) \mathbb{P}_{TND}(Y = 0\mid  \boldsymbol{C}  = \boldsymbol{c} )}{\mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c})};
\end{equation*}
\begin{equation*} 
     \mathbb{EIF}(\mu^0_v(\boldsymbol{c})) = \frac{\mathbb{I}\left(Y = 0, V= v,\boldsymbol{C}  = \boldsymbol{c}\right)-\mathbb{I}\left(V= v,\boldsymbol{C}  = \boldsymbol{c}\right) \mu^0_v(\boldsymbol{c})}{\mathbb{P}_{TND}(V= v,\boldsymbol{C}  = \boldsymbol{c})};
\end{equation*}
Thus, we have the EIF for $\omega_v(\boldsymbol{c}) = m^0(\boldsymbol{c})/\mu^0_v(\boldsymbol{c})$,
\begin{equation*} \label{2eifwetv2}
     \mathbb{EIF}(\omega_v(\boldsymbol{c}))  = \frac{ \mathbb{EIF}(m^0(\boldsymbol{c}))}{\mu^0_v(\boldsymbol{c})} - \frac{m^0(\boldsymbol{c})\mathbb{EIF}(\mu^0_v(\boldsymbol{c})) }{[\mu^0_v(\boldsymbol{c})]^2}. 
\end{equation*}

Term A in Equation (\ref{2EIFmost}) is:
\begin{align*}
    &\sum_{\boldsymbol{c}}\mathbb{EIF}(\mu_v(\boldsymbol{c}))\omega_v(\boldsymbol{c})\mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c}) \\ =& \sum_{\boldsymbol{c}} \frac{\mathbb{I}\left(Y = 1,V=v, \boldsymbol{C}  = \boldsymbol{c}\right)-\mathbb{I}\left(V=v,\boldsymbol{C}  = \boldsymbol{c}\right) \mu_v(\boldsymbol{c})}{\mathbb{P}_{TND}(V=v,\boldsymbol{C}  = \boldsymbol{c})} \omega_v(\boldsymbol{c})\mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c})  \\
    =& \sum_{\boldsymbol{c}} \frac{\mathbb{I}\left(Y = 1,V=v, \boldsymbol{C}  = \boldsymbol{c}\right)-\mathbb{I}\left(V=v,\boldsymbol{C}  = \boldsymbol{c}\right) \mu_v(\boldsymbol{c})}{\mathbb{P}_{TND}(V=v \mid \boldsymbol{C}  = \boldsymbol{c})} \omega_v(\boldsymbol{c}) \\
    =&\frac{\mathbb{I}(Y = 1, V=v)\omega_v(\boldsymbol{c}) - \mathbb{I}(V=v)\mu_v(\boldsymbol{c}) \omega_v(\boldsymbol{c})}{\pi_v(\boldsymbol{c})}\\
    =&\frac{\mathbb{I}(Y = 1, V=v)\omega_v(\boldsymbol{c}) }{\pi_v(\boldsymbol{c})} - \frac{\mathbb{I}(V=v)\mu_v(\boldsymbol{c}) \omega_v(\boldsymbol{c})}{\pi_v(\boldsymbol{c})}
\end{align*}
For Term B, to compute $\sum_{\boldsymbol{c}}\mu_v(\boldsymbol{c})\mathbb{EIF}(\omega_v(\boldsymbol{c}))\mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c})$, we first have
\begin{align*}
    &\sum_{\boldsymbol{c}}\mu_v(\boldsymbol{c}) \frac{ \mathbb{EIF}(m^0(\boldsymbol{c}))}{\mu^0_v(\boldsymbol{c})} \mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c}) \\ =& \sum_{\boldsymbol{c}}\mu_v(\boldsymbol{c}) \frac{ \mathbb{I}\left( Y=0, \boldsymbol{C}  = \boldsymbol{c}\right)-\mathbb{I}\left(\boldsymbol{C}  = \boldsymbol{c}\right) m^0(\boldsymbol{c})}{\mu^0_v(\boldsymbol{c})\mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c})} \mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c}) \\ 
    =& \frac{ \mathbb{I}(Y=0)\mu_v(\boldsymbol{c}) -\mathbb{I}( S=1) \mu_v(\boldsymbol{c})m^0(\boldsymbol{c})}{\mu^{0}_v(\boldsymbol{c})}    \\
    =& \frac{ \mathbb{I}(Y=0)\mu_v(\boldsymbol{c}) }{\mu^{0}_v(\boldsymbol{c})}   - \mathbb{I}( S=1)\mu_v(\boldsymbol{c})\omega_v(\boldsymbol{c});
\end{align*}
then we have
\begin{align*}
&-\sum_{\boldsymbol{c}}\mu_v(\boldsymbol{c})\frac{m^0(\boldsymbol{c})\mathbb{EIF}(\mu^0_v(\boldsymbol{c})) }{[\mu^0_v(\boldsymbol{c})]^2}\mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c}) \\ =&-\sum_{\boldsymbol{c}}\mu_v(\boldsymbol{c})\frac{m^0(\boldsymbol{c})\left\{ \mathbb{I}\left(V=v, \boldsymbol{C}  = \boldsymbol{c}, Y=0\right)-\mathbb{I}\left(V = v, \boldsymbol{C}  = \boldsymbol{c}\right) \mu^0_{v}(\boldsymbol{c})\right\} }{[\mu^0_v(\boldsymbol{c})]^2\mathbb{P}_{TND}(V=v, \boldsymbol{C}  = \boldsymbol{c})}\mathbb{P}_{TND}(\boldsymbol{C}  = \boldsymbol{c}) \\
=&- \sum_{\boldsymbol{c}}\mu_v(\boldsymbol{c})\frac{m^0(\boldsymbol{c})\left\{ \mathbb{I}\left(V=v, \boldsymbol{C}  = \boldsymbol{c}, Y=0\right)-\mathbb{I}\left(V = v, \boldsymbol{C}  = \boldsymbol{c}\right) \mu^0_{v}(\boldsymbol{c})\right\} }{[\mu^0_v(\boldsymbol{c})]^2\mathbb{P}_{TND}(V=v \mid \boldsymbol{C}  = \boldsymbol{c})} \\ 
=&- \mu_v(\boldsymbol{c})\frac{m^0(\boldsymbol{c})\left\{ \mathbb{I}\left(V=v, Y=0\right)-\mathbb{I}\left( V=v\right) \mu^0_{v}(\boldsymbol{c})\right\} }{[\mu^0_v(\boldsymbol{c})]^2\mathbb{P}_{TND}(V=v\mid \boldsymbol{C}  = \boldsymbol{c})}
\\ 
=&- \frac{\mu_v(\boldsymbol{c}) m^0(\boldsymbol{c})\left\{ \mathbb{I}\left(V=v, Y=0\right)\right\} }{[\mu^0_v(\boldsymbol{c})]^2\mathbb{P}_{TND}(V=v\mid \boldsymbol{C}  = \boldsymbol{c})} + \frac{\mu_v(\boldsymbol{c}) m^0(\boldsymbol{c})\left\{ \mathbb{I}\left( V=v\right) \mu^0_{v}(\boldsymbol{c})\right\} }{[\mu^0_v(\boldsymbol{c})]^2\mathbb{P}_{TND}(V=v\mid \boldsymbol{C}  = \boldsymbol{c})}
\\ 
=&- \frac{\mu_v(\boldsymbol{c}) m^0(\boldsymbol{c})\left\{ \mathbb{I}\left(V=v, Y=0\right)\right\} }{[\mu^0_v(\boldsymbol{c})]^2\mathbb{P}_{TND}(V=v\mid \boldsymbol{C}  = \boldsymbol{c})} + \frac{\mu_v(\boldsymbol{c}) \mathbb{I}\left( V=v\right)  }{\pi_v(\boldsymbol{c})} \omega_v(\boldsymbol{c})
\end{align*}

Plugging in the same results of Term C in the previous section, the EIF of $\psi_{v}$ can be expressed as follows:
\begin{align} \label{2EIFmost2V2}
    \mathbb{EIF}(\psi_{v}) &= \left[ \frac{\mathbb{I}(Y = 1, V=v) \omega(\boldsymbol{c})}{\pi_v(\boldsymbol{c})} + \frac{ \mathbb{I}(Y=0)\mu_v(\boldsymbol{c}) }{\mu^{0}_v(\boldsymbol{c})} - \frac{\mu_v(\boldsymbol{c}) m^0(\boldsymbol{c})\left\{ \mathbb{I}\left(V=v, Y=0\right)\right\} }{[\mu^0_v(\boldsymbol{c})]^2\mathbb{P}_{TND}(V=v\mid \boldsymbol{C}  = \boldsymbol{c})} \right] - \psi_{v} \nonumber \\
    &=\left[ \frac{\mathbb{I}(Y = 1, V=v)}{\pi^0_v(\boldsymbol{c})} - \omega_v(\boldsymbol{c})\mu_v(\boldsymbol{c})\left\{ \frac{ m^0(\boldsymbol{c})\mathbb{I}\left( V= v, Y=0\right) - \mathbb{I}\left(Y=0\right) \mu^{0}_v(\boldsymbol{c})\pi_v(\boldsymbol{c}) }{m^0(\boldsymbol{c})\mu^0_v(\boldsymbol{c})\pi_v(\boldsymbol{c})} \right\} \right] - \psi_{v} \nonumber \\
    &=\left[ \frac{\mathbb{I}(Y = 1, V=v)}{\pi^0_v(\boldsymbol{c})} - \omega_v(\boldsymbol{c})\mu_v(\boldsymbol{c})\left\{ \frac{\mathbb{I}\left( V= v, Y=0\right) - \mathbb{I}\left(Y=0\right) \mu^{0}_v(\boldsymbol{c})\pi_v(\boldsymbol{c})/ m^{0}_v(\boldsymbol{c})}{\mu^0_v(\boldsymbol{c})\pi_v(\boldsymbol{c})} \right\} \right] - \psi_{v} \nonumber \\
    &=\left[ \frac{\mathbb{I}(Y = 1, V=v)}{\pi^0_v(\boldsymbol{c})} - \omega_v(\boldsymbol{c})\mu_v(\boldsymbol{c})\left\{ \frac{ \mathbb{I}\left( Y=0\right) \left[\mathbb{I}(V=v) - \pi^0_{v}(\boldsymbol{c})\right] }{m^0(\boldsymbol{c})\pi^0_v(\boldsymbol{c})}  \right\}\right] - \psi_{v} \nonumber \\  &= \frac{\mathbb{I}(Y = 1, V=v)}{\pi^0_v(\boldsymbol{C})} - \mu_v(\boldsymbol{C})\left\{ \frac{ \mathbb{I}\left( Y=0\right) \left[\mathbb{I}(V=v) - \pi^0_{v}(\boldsymbol{C})\right] }{\pi^0_v(\boldsymbol{C})[1 - \mu_v(\boldsymbol{C})]}  \right\}  - \psi_{v} \nonumber \\
    & = \frac{\mathbb{I}(Y = 1, V=v) - odds_{TND}(Y \mid V=v,\boldsymbol{C})\mathbb{I}\left( Y=0\right) \left[\mathbb{I}(V=v) - \pi^0_{v}(\boldsymbol{C})\right]}{\pi^0_v(\boldsymbol{C})} - \psi_{v}, 
\end{align}
where the third and fourth equalities follow by the identity that $\omega_v(\boldsymbol{c})  = \pi_v(\boldsymbol{c}) / \pi^0_v(\boldsymbol{c})= m^0(\boldsymbol{c})/\mu^0_v(\boldsymbol{c})$, thus, $m^0(\boldsymbol{c})\pi^0_v(\boldsymbol{c}) = \mu^0_v(\boldsymbol{c})\pi_v(\boldsymbol{c})$ and $\pi^0_v(\boldsymbol{c}) = \mu^0_v(\boldsymbol{c})\pi_v(\boldsymbol{c})/m^0(\boldsymbol{c})$, and again, the specific form of $\omega(\boldsymbol{c}) = [1 - m(\boldsymbol{c})]/[1 - \mu_v(\boldsymbol{c})]$ leads to the equation in the last second, $odds_{TND}(Y \mid V=v,\boldsymbol{C})$ in the last equation is the odds under $\mathbb{P}_{TND}$ of $Y=1$ given $V=v$ and $\boldsymbol{C}$.

In Equation (\ref{2EIFmost2}), the EIF for $\psi_v$ is derived by debiasing weights in the form of a propensity ratio, whereas in Equation (\ref{2EIFmost2V2}), the EIF is derived by debiasing weights in the form of an outcome probability ratio. As anticipated, the results derived from these two different processes are mathematically identical. 


